SIMARA: a database for key-value information extraction from full pages

We propose a new database for information extraction from historical handwritten documents. The corpus includes 5,393 finding aids from six different series, dating from the 18th-20th centuries. Finding aids are handwritten documents that contain metadata describing older archives. They are stored in the National Archives of France and are used by archivists to identify and find archival documents. Each document is annotated at page-level, and contains seven fields to retrieve. The localization of each field is not available in such a way that this dataset encourages research on segmentation-free systems for information extraction. We propose a model based on the Transformer architecture trained for end-to-end information extraction and provide three sets for training, validation and testing, to ensure fair comparison with future works. The database is freely accessible at https://zenodo.org/record/7868059.

==> simara_application.tex <==
It may be useful to explain by now how the SIMARA system works. SIMARA is a front-end leaned back on a HTR and NER infrastructure (see fig.\,\ref{fig:schema_simara} below). This interface is used by the National Archives to upload their data, mainly the pictures of the digitized finding aids, but also to help Teklia training the models and improve them. We will sum up briefly the process of conversion of a finding aid.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/simara_schema.png}
    \caption{Functional schema of SIMARA.}
    \label{fig:schema_simara}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_5.png}
    \caption{Annotator view: typing ground truth (transcription of the information into the corresponding fields of the form).}
    \label{fig:interf_simara_5}
\end{figure}


\subsection{Supplying groundtruth}

%!! Paragraphe à réécrire et corriger sans doute !! Je sors de ma partie...%%
It was necessary at the beginning of the project to create groundtruth data, as the writings were very different. We tried to create a global model that could handle all this diversity of scriptings. Today it may be necessary to supply groundtruth data in new projects if the writings are very different or if the model needs to be improved.


The SIMARA interface is mainly used by two kind of users: the "archivists" and the "annotators", which are the two main roles an user can have -- excepted the administrators. The archivists manage the conversion of the handwritten finding aid. The annotators have an important role as they supply groundtruth data by typing the text of the original finding aid, or read and correct the transcriptions made by the artificial intelligence. The pictures below are screenshots taken from the SIMARA interface at the main steps of the process.

\subsection{Creating a project for a finding aid}

The "archivist" user has to create a project for each finding aid. Here is his landing page where he can see all the current projects (fig.\,\ref{fig:interf_simara_1}).

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_1.png}
    \caption{Archivist view: list of the projects (finding aids currently handled).}
    \label{fig:interf_simara_1}
\end{figure}

\subsection{Building a form}
The "archivist" also identifies all the categories into which the information of the finding aid can be spread. These correspond to the cases seen above in the section \ref{section_simara_dataset}: see for instance the example of the X series, p.\,\pageref{information_example}. He will build accordingly to this analysis a form that contains fields corresponding to an XML EAD element. For instance, the date of a record will be handled by the "Date" field, which corresponds to the $<$unitdate$>$ XML EAD element. The fig.\,\ref{fig:interf_simara_2} below represents the step of form building.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_2.png}
    \caption{Archivist view: creating a form for a finding aid (categories of information, related to an XML EAD element).}
    \label{fig:interf_simara_2}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_3.png}
    \caption{Archivist view: distributing tasks to different annotators.}
    \label{fig:interf_simara_3}
\end{figure}

On his landing page, the "annotator" can see all the projects he is involved in (fig. \ref{fig:interf_simara_4}).

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_4.png}
    \caption{Annotator view: list of projects he is involved in.}
    \label{fig:interf_simara_4}
\end{figure}


Typing the content of a record is a "task" (see fig. \ref{fig:interf_simara_5} below). The archivist, as the manager of the project spreads the tasks between several "annotators" (fig.\,\ref{fig:interf_simara_3}).

Another kind of tasks the "annotator" has to deal with is reading the automatic transcriptions generated by artificial intelligence. Thanks to the use of HTR and NER processes, the contents of the finding aid are transcribed and put into the fields of the form. Once the transcriptions are put into SIMARA, the "annotator" can begin to read, confirm and correct the text.

\subsection{The case of registers finding aids}
The examples shown till here are file finding aids, that is files constituted of individual cards, each card corresponding to a document or an act. There are also finding aids written on registers. This kind of document has to be handled differently as on a same page you can find several records. They need to be identified, and the "annotator" that has to supply groundtruth has also to draw each record on the page, to help artificial intelligence to segment the page (fig.\,\ref{fig:interf_simara_6}).

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_6.png}
    \caption{Annotator view: list of annotation zones (on a register finding aid: several records are written on the same page).}
    \label{fig:interf_simara_6}
\end{figure}

Once these zones are drawn, the "annotator" can fill in the form as usual (fig.\,\ref{fig:interf_simara_7}).

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_7.png}
    \caption{Annotator view: typing ground truth of a zone on a register finding aid.}
    \label{fig:interf_simara_7}
\end{figure}

\subsection{Retrieve the XML code from SIMARA}
The final step for the archivist is to retrieve from the SIMARA solution a complete and well-formed XML EAD document, that will be then uploaded into the information system of the National Archives, so that the digital finding aid can be published and available on the Internet. The constraints of the DTD used by the National Archives have been taken into account; consequently, all the information present into the fields of the form are written into XML.

The archivist has the possibility to control and correct the work of the "annotators". He can preview the result of the encoding of each record (fig.\,\ref{fig:interf_simara_8}), but of course can also download the whole XML finding aid.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/interface_simara_8.png}
    \caption{Archivist view: verifying the XML formalism after the text was transcribed and corrected by an annotator.}
    \label{fig:interf_simara_8}
\end{figure}


